How to Teach DNNs to Pay Attention to the Visual Modality in Speech Recognition

Audio-Visual Speech Recognition (AVSR) seeks to model, and thereby exploit, the dynamic relationship between a human voice and the corresponding mouth movements. A recently proposed multimodal fusion strategy, AV Align, based on state-of-the-art sequence to sequence neural networks, attempts to model this relationship by explicitly aligning the acoustic and visual representations of speech. This study investigates the inner workings of AV Align and visualises the audio-visual alignment patterns. Our experiments are performed on two of the largest publicly available AVSR datasets, TCD-TIMIT and LRS2. We find that AV Align learns to align acoustic and visual representations of speech at the frame level on TCD-TIMIT in a generally monotonic pattern. We also determine the cause of initially seeing no improvement over audio-only speech recognition on the more challenging LRS2. We propose a regularisation method which involves predicting lip-related Action Units from visual representations. Our regularisation method leads to better exploitation of the visual modality, with performance improvements between 7% and 30% depending on the noise level. Furthermore, we show that the alternative Watch, Listen, Attend, and Spell network is affected by the same problem as AV Align, and that our proposed approach can effectively help it learn visual representations. Our findings validate the suitability of the regularisation method to AVSR and encourage researchers to rethink the multimodal convergence problem when having one dominant modality.

==> author_info/author_bios.tex <==
George Sterpu received the BS degree in systems engineering from University Politehnica of Bucharest, Romania, in 2013, and the MS degree in automation and control theory from University Grenoble Alpes, France, in 2015. He is currently pursuing a PhD in Audio-Visual Speech Recognition at Trinity College Dublin, Ireland.

Christian Saam received an M.A. degree in computational linguistics and phonetics from Trier University, Trier, Germany in 2001. From 2009 to 2013, he was a Research Assistant at Karlsruhe Institute of Technology and from 2013 to 2015 at Trinity College Dublin. Since 2015, he has been a Research Fellow at ADAPT Centre, Trinity College Dublin.
His research interests include automatic speech recognition, speech processing, multi-modality, natural language processing and dialog modelling.

Naomi Harte is an Associate Professor in the School of Engineering, Trinity College Dublin, Ireland. She leads a major national research strand in multimodal interaction at the ADAPT SFI Centre in Ireland. Her research interests include audio-visual speech recognition, conversation analysis, speech synthesis evaluation and birdsong.

